Task Arithmetic can Mitigate Synthetic-to-Real Gap in Automatic Speech Recognition

Synthetic data is widely used in speech recognition due to the availability of text-to-speech models, which facilitate adapting models to previously unseen text domains. However, existing methods suffer in performance when they fine-tune an automatic speech recognition (ASR) model on synthetic data as they suffer from the distributional shift commonly referred to as the synthetic-to-real gap. In this paper, we find that task vector arithmetic is effective at mitigating this gap. Our proposed method, SYN2REAL task vector, shows an average improvement of 10.03\% improvement in word error rate over baselines on the SLURP dataset. Additionally, we show that an average of SYN2REAL task vectors, when we have real speeches from multiple different domains, can further adapt the original ASR model to perform better on the target text domain.

==> sections/4_1-method.tex <==
\section{Methodology}
\label{sec:method}
In this work, we aim to adapt ASR models from source domains with real speech and text data to a new domain with only text data. More specifically, we adapt ASR models using data synthesized from off-the-shelf text-to-speech (TTS) models.
However, ASR models often perform poorly due to acoustic differences between synthetic data generated by TTS and real speech data. To overcome this limitation, we introduce the \method task vector, a novel approach that bridges the gap between the acoustic characteristics of synthetic and real speech data.

\subsection{Domain Mismatch in ASR Domain Adaptation}


\subsection{Problem Formulation}
We assume a problem setting in which we have two domains: a source domain $D_s$ and a target domain $D_t$. 
%, where $D_s, D_t \subset D$. 
The source domain $D_s$ consists of paired text and speech samples, denoted as $T_s$ and $S_s$, respectively. The target domain $D_t$ contains only text data, denoted as $T_t$. This problem setting is common as it is easy to generate synthetic text data, whereas collecting paired real speech data is labor-intensive.% This work aims to adapt ASR models to the target domain using only text data from $D_t$ without access to corresponding real speech samples.

\subsection{\method Task Vector}
To adapt ASR models to a previously unseen domain, we employ a common methodology \cite{joshi-singh-2022-simple} that utilizes synthetic data generated from the target text $T_t$ for model adaptation. 
%As depicted in Figure~\ref{fig:method}, we utilize a model to generate synthetic speech from the target text $T_t$. The synthetic speech is then used to fine-tune the ASR model, facilitating domain adaptation to the target domain.

% \subsection{\method Task Vector}

\begin{figure}[htp!]
\begin{adjustbox}{width=\linewidth}
\centering
\includegraphics{pics/method.drawio.pdf}
\end{adjustbox}
\caption{\textbf{Framework for \method task vector in Domain Adaptation for ASR.} The framework illustrates the process of creating the \method task vector by subtracting the parameter differences between a model fine-tuned on synthetic speech (Source Synthetic) and a model fine-tuned on real speech (Source Real) from pretrained ASR (PASR). This task vector is then applied to the target synthetic domain (Target Synthetic) to improve ASR performance by bridging the gap between synthetic and real speech data.}
\label{fig:method}
\end{figure}

Previous work in task arithmetic has demonstrated that vectors can encode distinct capabilities, such as language or domain-specific features. We hypothesize that the differences in acoustic properties between real and synthetic speech are also learnable and can be isolated through parameter arithmetic. Specifically, we assume that we have models fine-tuned on real and synthetic data from the source domain, denoted as $\theta_{real}^{S}$ and $\theta_{syn}^{S}$ respectively.
The acoustic disparity between real and synthetic speech is quantified by subtracting the parameter sets of these models:
\begin{equation}
\tau = \theta_{real}^{S} - \theta_{syn}^{S}
\end{equation}

Once the \method vector $\tau$ is computed, we apply it to the model parameters fine-tuned on the synthetic data in the target domain, $\theta_{syn}^{T}$, thereby enhancing its adaptation to the target domain:
\begin{equation}
\theta_{syn\_new} = \theta_{syn}^{T} + \lambda \tau
\end{equation}
Where $\lambda$ is the scaling factor of \method task vector.

This adjusted model, $\theta_{syn\_new}$, is expected to perform more robustly in the target domain as it incorporates the acoustic characteristics of real speech, making it better suited for practical ASR tasks where real speech is present.

%\paragraph{Alternative \method Task Vector Formulation}
%%% Extending this to scneaiors where we have access to data in muliple domains
\paragraph{\methodd}
In the previous discussion, we assume no access to domain labels such as 'email' or 'music' from the source domain to emulate real-world situations better. All real speech data falls in the source domain. 
% Therefore, we formulated the \method task vector as the weight difference between \sun{TODO} after training the ASR on data, jointly.
%wby training the ASR model on the source domain data jointly. 
In scenarios where we have access to data of multiple domains, another approach is to create \method task vectors for each domain separately and then combine these vectors. This method involves fine-tuning separate ASR models on each individual source domain to obtain domain-specific \method task vectors, which are then averaged to form a comprehensive \method task vector.

For each domain $i$ in source domain $S$. The task vector can be defined as:
\begin{equation}
\tau_i = \theta_{real}^{S_i} - \theta_{syn}^{S_i}
\end{equation}
Where  $\theta_{real}^{S_i}$ and $\theta_{syn}^{S_i}$ represent the model parameters fine-tuned on real and synthetic data for domain $i$ respectively.
Once the vector $\tau_i$ is computed, we apply it to the model parameters fine-tuned on synthetic target domain data $\theta_{syn}^{T}$, thereby enhancing its adaptation to the target domain:
\begin{equation}
\theta_{syn\_new} = \theta_{syn}^{T} + \frac{\lambda}{|S|} \sum_{i=0}^{|S|} \tau_i
\end{equation}
Where $|S|$ is the number of source domains, and $\lambda$ is the scaling factor for the task vector.
%While this alternative approach could potentially capture more detailed domain-specific characteristics, it relies on the availability of explicit domain labels, which may not always be present in real-world situations. In practice, the absence of domain labels makes it challenging to apply this method effectively, as it would require additional steps to infer or estimate the domain of each data sample.
%Considering real-world applications, the joint training approach without source domain labels is more feasible and practical, as it does not depend on domain labels and can generalize better across various domains. However, we still show the experiments of the setting with source domain labels and discuss in Section~\ref{sec:dis}.
